Airlock: Bounding the Multi-Agent Blast Radius via Selective Online Containment

When multi-agent systems act on the external world, a single agent's faulty output can spread across tasks before detection, creating a system-wide blast radius. Single-agent guardrails are confined to individual harnesses, while existing multi-agent controls either cancel only the faulty source and miss downstream consumers or halt and roll back the entire workflow at the cost of healthy work. We present Airlock, a multi-agent runtime and guardrail for selective post-alert fault containment. Its tree-structured runtime, EdgeCitadel, narrows permissions vertically from parent to child agents to establish node boundaries and control switches. Meanwhile, an append-only provenance DAG records cross-agent data consumption horizontally. Upon an alert, Airlock traces forward on this DAG to isolate tainted executions and pending actions, and backward to narrow root causes. At the site switches, a default full quarantine tier freezes affected branches without a solver, while an assured optimized cut tier uses fence-then-prune to enforce a deadline-aware minimum cut minimizing collateral disruption. Across 1,832 testbed runs, 161 physical smart-home LLM runs, and 24,266 simulation records, Airlock blocks all post-alert faulty actuations on our main testbed and smart-home grids with zero post-convergence leaks. Whereas native controls in A2A and LangGraph either contain at most 33.3% of faults or retain at most 16% of work without redo, Airlock retains +68 pp to +96 pp more healthy work, and its optimized cut retains +46 pp more than full quarantine under dense spread. These results show that co-designing runtime authority boundaries with online provenance enables surgical fault containment without sacrificing healthy work (code: https://github.com/EdgeCitadelTeam/EdgeCitadel).

==> sections/app-c-amend.tex <==
\paragraph{Registered after 2026-10-22,} each before any run of its grid.
\begin{itemize}
\item[] H13 (detector grid, 2026-10-23). Two harness-only faults make the faulty invocation cross a boundary, an out-of-scope dispatch (refused at admission) and a deadline runaway (expired by its lease), on C2 and rand-n7-s1 with no injected alert (36 faulted runs, 6 references). H13a: every faulted run is detected by the authority or the resource boundary detector, naming the faulty invocation; median detection latency $\le$ 500~ms per class and every run $\le$ 1,500~ms; no detector incident in a reference run or before the lineage's alert. H13b: a decision $\le$ 0.2~s after the detector alert; \FB commits no tainted effect after $\tone$ in any run and reaches $\tone$ within 2.0~s in $\ge$ 90\% of runs; \FB and Trace \& quarantine are clean after the alert in every run, No containment in none; the ranked root includes the faulty invocation in $\ge$ 90\%; kept work is reported only. H13c: effect-level violations are refused at the gateway but open no incident; stated, not tested.
\item[] H14 (control-delay grid, 2026-10-24). C2 and N2, five controls, 1~s and 4~s of added control delay with $L$ = the added delay + 400~ms (132 runs). H14a (confirmatory): no tainted effect commits after $\tone$ in any run of the three cut strategies at either delay; a run without $\tone$ or one that timed out counts against it. H14b: the clean rate after the alert does not rise with delay; \FB's freeze rate rises and its kept work does not. H14c: at 4~s \FB keeps at least as much work as Cut without deadlines and as Greedy cut on matched runs (one-sided sign-flip tests, $\alpha = 0.05$ each). H14d: \FB against Trace \& quarantine, descriptive. The main runs' deadline ablation was known at registration.
\item[] H15 (full quarantine in the system comparison's rogue cells, 20 runs, 2026-10-24). H15a: cut mode's clean rate is at least quarantine mode's and its tainted commits at most quarantine mode's on matched runs (one-sided Fisher exact and paired sign-flip tests, $\alpha = 0.05$). H15b: kept work, two-sided and descriptive, with the simulator's prior that quarantine mode keeps about 1 percentage point more. Known at registration: the comparison's \FB rows and the main runs' rogue-0.3 rows, in which both settings were clean in every run.
\item[] H16 (meeting rooms, 2026-10-24, before the physical pilot; decided on the formal runs). H16a (confirmatory): in every run in which the wrong booking is consumed, at either injection point, full quarantine and the optimized cut commit no wrong physical effect after the alert (the optimized cut also none after $\tone$), and No containment commits at least one in most consumed runs. H16b (one-sided, the optimized cut only): $\tone \le 1.0$~s. H16c to H16f are descriptive. H16g (confirmatory, physical): every physical change seen by the camera or the lamps' read-back has a ledger commit, and held effects show none. Five amendments (2026-10-25 and 26) fixed the setup: a session-isolated calendar, frozen code, the device credential kept on one host, gateway rate limits, a camera settle time, a night slot for the API models (H16g reported per slot) and the API grid size.
\emph{Outcome:} H16a holds on the Qwen runs (\fact{F-T567} and \fact{F-T572} wrong effects after the alert at the two points, \fact{F-T676} after $\tone$, and No containment at least \fact{F-T673} and \fact{F-T674} per run), and H16b holds (largest $\tone$ \fact{F-T677}); in the mixed deployment, not pooled, one run's $\tone$ is \fact{F-T654}. H16g is not decided as registered: none of the marks its check counts was written (\fact{F-T697} in \fact{F-T704} runs) and the read-back was not recorded. Post hoc, against the lamps' Home Assistant history, every lamp change during the runs followed a gateway commit and no held command changed a lamp (Section~5.2).
\item[] H12 (scaled testbed, 2026-10-24). H12a (confirmatory): no tainted effect commits after $\tone$ in any optimized-cut run at any reported site count; runs without $\tone$, timeouts and fallback alerts count against it. H12b (one-sided): a decision within 2.0~s. H12c to H12g are descriptive; H12-sim compares with the simulator at 32 sites, its prediction filed before any scale run.
\emph{Outcome.} H12-A2 (2026-10-27, before the rerun's first run) reruns the optimized-cut cells on the released build with the same cells, seeds and run identifiers and supersedes the original runs. No run reached $\tone$ within its window (\fact{F-E169} of \fact{F-E168}), so H12a fails; \fact{F-E171} of \fact{F-E168} runs was clean after the alert. Within the runs no hold was released (\fact{F-E173}), no decision was contained without $\tone$ (\fact{F-E176}) and one alert was deferred (\fact{F-E174}). The rerun's registered replay check is not met as registered: it flags \fact{F-E175} releases, all \fact{F-E180} to \fact{F-E181} after the run's end and \fact{F-E177} before it, while a post-hoc check finds every flagged action covered by the fence positions of the converged record before its release (\fact{F-E185} of \fact{F-E184}, \fact{F-E186} uncovered).
\end{itemize}

\paragraph{Amendments, in date order.}
\begin{itemize}
\item[] \emph{HomeSvc early alert} (2026-10-21, before the pilot). With faster hand-offs a 0.3~s delay could fall after the assistant's read, so the alert now fires on the produce event; whether the schedule was read at the alert is recorded.
\item[] \emph{Control latency} (2026-10-22, after the pilot). The pilot's confirmation tails exceeded the planned $L = 150$~ms, so every native regime after it plans with $L = 400$~ms at every site; the pilot is not reported.
\item[] \emph{Kept-work metric} (2026-10-22, before any main-run result was scored). A refused hand-off into the declared tainted closure no longer makes a healthy task incomplete: the cuts refuse such hand-offs, while full quarantine and A2A pause the consumer, so the same clean work was scored lost under one and kept under the other. Re-score only, for every control and grid; on the pilot every changed cell moved up.
\item[] \emph{Re-executed work} (H10-LG; 2026-10-22, before any LangGraph run). A task started again after the alert counts as redone, for every system; time travel's kept-work prediction is withdrawn and reported only.
\item[] \emph{H13's kept-work clause} (2026-10-23, at registration). The draft's one-sided test against Trace \& quarantine became descriptive, because the pilot showed a kept-work gap that the frozen design does not close; a local dry run of the detector grid preceded registration.
\item[] \emph{Saturated-rogue cells of H10 and H10-LG} (2026-10-23; for H10 after its grid ran, no run repeated). At rogue rate 1.0 our runtime's authority detector alerted before the injected alert's trigger, while A2A and LangGraph receive only the injected alert, so these runs are scored from the earliest alert on the fault's lineage and reported separately; the registered tests are unchanged.
\item[] \emph{H8, correct answers} (2026-10-24, before the HomeSvc runs were scored). A wrong answer from the contaminated assistant had counted as service; HomeSvc now reports correct and wrong answers, and the service claim uses correct answers. H8 is still decided as registered.
\item[] \emph{H10-LG, reduced grid} (2026-10-24, before any LangGraph run). 129 runs replace 269 (C2, C3 and rand-n7-s1; 3 repetitions); thresholds unchanged; the Fisher test of (ii) has $n = 6$ per control.
\item[] \emph{Control-delay grid} (2026-10-24, with H14). It replaces the earlier stress grid; $L$ is the added delay plus 400~ms instead of the delay.
\item[] \emph{H12-A1, a deviation} (2026-10-25, after the 3- and 8-site runs, before any run at 16 or 63 sites). The curve became 16, 32 and 63 sites: at 3 and 8 sites worker slots restarted, from the agent daemon's default listen backlog of 5, and the no-fault references did not complete. Because the drop removes probable counterexamples to H12a, we report it as a deviation.
\item[] \emph{Fenced $\tone$ (scoring)} (2026-10-25, before any re-score and before the audit's output was read). $\tone$ is the first converged record of the incident at which every action in force for that incident, from all its decisions, is fenced; a run without it has no $\tone$. It applies to every grid and is at least as strict as Theorem~5's check. \emph{Reason:} the implemented check fenced only the current decision's new actions, so a re-solve that applied nothing could log a vacuous $\tone$. \emph{Audit:} the registered audit counted \fact{F-T511}, \fact{F-T512}, \fact{F-T513} and \fact{F-T514} runs with a fenced $\tone$ in the main, HomeSvc, system-comparison and control-delay grids (\fact{F-T509} in all) and none unfenced outside the scaled testbed (\fact{F-T510}), but it read only records logged before each converged record (\fact{F-T801}). A corrected audit, post hoc, collects every action of the incident: of the \fact{F-T800} main-grid runs with a $\tone$, \fact{F-T797} are fenced with at least one action in force, \fact{F-T798} have no action of the operator's incident in force and \fact{F-T799} are unfenced, so every main-grid $\tone$ stands. In \fact{F-T802} of the \fact{F-T798} nothing tainted was live; in the other \fact{F-T805} the operator's solve chose only actions already in force under the detector's earlier incident, all fenced before $\tone$. The scaled testbed's logged $\tone$ were unfenced; those runs are superseded (H12).
\item[] \emph{Procedure only} (2026-10-21 and 22). Hand-off speed and control latency are recorded instead of blocking a run, and the main runs' gate blocks on any tainted commit after $\tone$; ``alert timing'' became detection delay; after a host lost power the system comparison ran before the HomeSvc runs; the main and comparison grids wait up to \conf{10~s}{harness} for the coordinator to know the faulty invocation before alerting.
\item[] \emph{Not amended.} H11 is reported as registered. No other hypothesis or threshold changed after its registration.
\end{itemize}

